A Maximum Matching Algorithm for Basis Selection in Spectral Learning

We present a solution to scale spectral algorithms for learning sequence functions. We are interested in the case where these functions are sparse (that is, for most sequences they return 0). Spectral algorithms reduce the learning problem to the task of computing an SVD decomposition over a special type of matrix called the Hankel matrix. This matrix is designed to capture the relevant statistics of the training sequences. What is crucial is that to capture long range dependencies we must consider very large Hankel matrices. Thus the computation of the SVD becomes a critical bottleneck. Our solution finds a subset of rows and columns of the Hankel that realizes a compact and informative Hankel submatrix. The novelty lies in the way that this subset is selected: we exploit a maximal bipartite matching combinatorial algorithm to look for a sub-block with full structural rank, and show how computation of this sub-block can be further improved by exploiting the specific structure of Hankel matrices.

==> faster-sup.tex <==

\begin{figure*}[t]
  \begin{center}
  \includegraphics[width=\linewidth]{speedupMatching-aistats.pdf}%
\end{center}
  \caption{Average and standard deviation (10 iterations) of the time spent for the baseline (in blue) and our proposed solution (in red). $x$-axis is the number of sequences, $y$-axis time in seconds.}
    \label{fig:speedup}
\end{figure*}


\section{Synthetic Experiments for the Fast Augmenting Path Algorithm}

A theoretical analysis of the Fast Augmenting Path Algorithm
(presented in Section 4 of the main paper) is challenging. While each
iteration is never worse than the baseline iteration (the checks can
be done in time $\BigO{|E|}$ assuming a bitset implementation of
sets), it may well be that none of the shifted pairs are free, and
therefore only add computation without improving the matching.

We therefore compared its execution time empirically on synthetic
data. Random sequences were generated with different alphabet size,
and different average length (we sampled from a Gaussian distribution
with a variance of $0.5$).  The respective times are plotted in
Figure~\ref{fig:speedup} for different alphabet sizes ($|\Sigma|$) and
mean lengths ($\mu_{\textit{length}}$).

The proposed solution is always better, with increased speed-up with
increasing mean length (the average speed-up over all plots goes from
$1.18$ to $2.66$), and with a smaller slope.  Both implementations are
probably sub-optimal and done in \texttt{python}.  However, we believe
these conclusions carry on to more sophisticated implementations, as
any improvement will affect both versions (arguably not equally, as
the baseline runs the augmenting path procedure more often).



==> related.tex <==



\section{Related Work}

In this section we describe the most popular alternative solutions to
the problem of scaling the spectral method.

\begin{itemize}

\item \textbf{Sparse SVD (SSVD):} A natural approach to deal with
  sparse function is to perform the SVD using an algorithm optimized
  for sparse matrices. One popular approach is to use variations of
  Lanczos algorithm which is what standard packages such as LAPACK
  implement for sparse singular value decomposition. In our
  experiments we will consider this as a baseline
  \citep{ssvd_1,ssvd_2}.
\item \textbf{High norm rows and columns (HN):} Another common
  approach to perform SVD of large matrices is based on sampling rows
  and columns of high norm \citep{sampling}.
\item \textbf{ Randomized Projections (RP):} In the context of Hankel
  based methods the dominant approach for dealing with large matrices
  has been to use SVD routines based on randomized projections
  \citep{rp_1,rp_2}.
\end{itemize}


%\end{itemize}


%-- below is more for other sections
%-- Volumme sampling is NP hard (get reference) we do something different.!!!!
%-- It has been shown that statistically it makes sense to use the complete hankel.
%This hankel becomes very very large.

This paper's novelty hinges on exploiting an efficient graph-based
combinatorial algorithm to perform sub-block selection of large and
sparse Hankel matrices. Our experiments show that our method is
significantly more efficient than state of the art approaches for
scaling spectral methods for the estimation of minimal WAs . Standard
packages for solving sparse linear systems do sometimes implement best
bipartite matching algorithms as a preprocessing step. However, to the
best of our knowledge, best matching algorithms have not been used in
the context of scaling Hankel based methods for the estimation of
sparse sequence functions.


